Feature Clock: High-Dimensional Effects in Two-Dimensional Plots

Humans struggle to perceive and interpret high-dimensional data. Therefore, high-dimensional data are often projected into two dimensions for visualization. Many applications benefit from complex nonlinear dimensionality reduction techniques, but the effects of individual high-dimensional features are hard to explain in the two-dimensional space. Most visualization solutions use multiple two-dimensional plots, each showing the effect of one high-dimensional feature in two dimensions; this approach creates a need for a visual inspection of k plots for a k-dimensional input space. Our solution, Feature Clock, provides a novel approach that eliminates the need to inspect these k plots to grasp the influence of original features on the data structure depicted in two dimensions. Feature Clock enhances the explainability and compactness of visualizations of embedded data and is available in an open-source Python library.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> figures/rotationTikz.tex <==

% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{figures/rotation.pdf}
% \caption{Rotation of the coordinate system}
% \label{fig:coordinateRotation}
% \end{figure}


==> figures/teaser_old.tex <==


\tikzset{HDnodeBase/.style={draw=gray!50!white,fill=red, minimum height=6, minimum width=5, inner sep=0.0}}
\tikzset{HDnodeBlue/.style={HDnodeBase,fill=mplBlue}}
\tikzset{HDnodeRed/.style={HDnodeBase,fill=mplRed}}
\tikzset{HDnodePink/.style={HDnodeBase,fill=mplPink}}
\tikzset{HDnodeGreen/.style={HDnodeBase,fill=mplGreen}}
\tikzset{HDnodeCyan/.style={HDnodeBase,fill=mplCyan}}
\tikzset{HDnodeOrange/.style={HDnodeBase,fill=mplOrange}}
\tikzset{HDnodeOlive/.style={HDnodeBase,fill=mplOlive}}
\tikzset{HDnodeBrown/.style={HDnodeBase,fill=mplBrown}}
\tikzset{HDnodeGray/.style={HDnodeBase,fill=mplGray}}
\tikzset{HDnodeGray/.style={HDnodeBase,fill=mplGray}}
\tikzset{HDnodePurple/.style={HDnodeBase,fill=mplPurple}}

\tikzset{roundnode/.style={circle, draw=mplPink!60, fill=mplPink!5, very thick, minimum size=4mm, inner sep=0.0, font=\rmfamily,yshift=0.5cm}}

\newcommand{\nodeLabel}[1]{
    \begin{tikzpicture}[]
        \node[roundnode, minimum size=2mm]{\fontsize{5}{5}\selectfont{#1}};
    \end{tikzpicture}
}


\centering
\vspace{-0.5cm}
\begin{tikzpicture}[]
    \begin{scope}[yshift=0.4cm]
        \begin{scope}[xshift=-1.2cm] %HD
        \node[roundnode, xshift=-1.1cm]{a};
        \node[font=\rmfamily,yshift=0.8cm,anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c}High dim. data \textbf{X}\end{tabular}}};

        \foreach \i in {1,...,21}
        {
            \pgfmathtruncatemacro{\y}{(\i - 1) / 7};
            \pgfmathtruncatemacro{\x}{(\i - 7 * \y)};
            \ifthenelse{\x = 1}{\node[HDnodeBlue]   at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 2}{\node[HDnodeRed]    at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 3}{\node[HDnodeGreen]  at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 4}{\node[HDnodePurple] at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 5}{\node[HDnodeGray]   at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 6}{\node[HDnodePink]   at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
            \ifthenelse{\x = 7}{\node[HDnodeOrange] at (0.21 * \x-0.84, 0.25 * \y + 0.25) {};}{}
        }
    \end{scope}

    \begin{scope}[yshift=-0.9cm,xshift=-1.2cm] %LD
        \node[font=\rmfamily,yshift=0.5cm, anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c} Low dim. data \textbf{Y} \end{tabular}}};

        \foreach \i in {1,...,6}
        {
            \pgfmathtruncatemacro{\y}{(\i - 1) / 2};
            \pgfmathtruncatemacro{\x}{(\i - 2 * \y)};
            \ifthenelse{\x = 1}{\node[HDnodeBrown]   at (0.21 * \x-0.21, 0.25 * \y) {};}{}
            \ifthenelse{\x = 2}{\node[HDnodeCyan]    at (0.21 * \x-0.21, 0.25 * \y) {};}{}
        }
    \end{scope}    
    \end{scope}
    

    \begin{scope}[xshift=1.5cm] %beta0
        \node[roundnode, xshift=-0.65cm, yshift=0.8cm]{b};
        \node[font=\rmfamily,yshift=0.8cm, xshift=0.9cm, anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c} Define optimization \\ problem \end{tabular}}};
        \node[font=\rmfamily,anchor=south,xshift=0.1cm,yshift=-0.4cm]{\fontsize{8}{8}\selectfont{
        \setlength\tabcolsep{0.pt}%
        \begin{tabular}{rl} 
        {\color{violet}$\mat{y_\theta}$} &$= \mat{X}\beta_\theta$ \\[0.17cm]
        $\theta^j$ &$= \argmaxF_{\theta \in [0..180\degree)} \lvert\beta^j\rvert$ \\[-0.07cm]
        \end{tabular}
        }};

         \begin{scope}[scale=1.6, xshift=.9cm, yshift=-0.1cm]
            \draw [gray,-{Latex[length=1.5mm]}, line width=0.2mm] (-0.1,0) -- (0.85,0);
            \draw[gray,-{Latex[length=1.5mm]}, line width=0.2mm] (0,-0.1) -- (0,0.6);

            % \draw [gray,dotted, line width=0.16mm] (0,0.4) -- (0.7,0.4);
            % \draw[gray,dotted,line width=0.16mm] (0.7,0) -- (0.7,0.4);
    
            % \draw[mplCyan,-{Latex[length=2mm]}, line width=0.5mm] (0,0) -- (0,0.4);
            % \draw[mplBrown, -{Latex[length=2mm]}, line width=0.5mm] (0,0) -- (0.7,0.0);
            % \draw[line width=0.5mm] (-0.00,-0.00) -- (0.7,0.4);
            \draw[line width=0.3mm, dashed] (-0.07,-0.04) -- (0.77,0.44);
            % \node[anchor=south east] at(0.77,0.44){\fontsize{8}{8}\selectfont{$y_\theta$}};
            
            \draw[thick, ]
            (0.2296,0) .. controls (0.2277,0.0519)..
            (0.1890,0.0945);
            \node[anchor=west] at(0.3277,0.119){\fontsize{8}{8}\selectfont{$\theta$}};
            \draw[gray] (0.15,0.55)            -- (0.35,0.2);
            \draw[gray] (0.7+0.044,0.4-0.077)  -- (0.7,0.4);
            \draw[gray] (0.7-0.21-0.088,0.4-0.12+0.14) -- (0.7-0.21,0.4-0.12);
        
            \filldraw[violet] (0.35,0.2) circle (1pt);
            \filldraw[violet] (0.7,0.4) circle (1pt);
            \filldraw[violet] (0.7-0.21,0.4-0.12) circle (1pt);

            \filldraw[gray] (0.15,0.55) circle (1pt);
            \filldraw[gray] (0.7+0.066,0.4-0.0955) circle (1pt);
            \filldraw[gray] (0.7-0.21-0.088,0.4-0.12+0.14) circle (1pt);
            
        \end{scope}
    \end{scope}

    \begin{scope}[xshift=1.5cm] %beta90
    \end{scope}

    \begin{scope}[xshift=10cm] %Filter $\beta_{i\degree}^j$
        \node[roundnode, xshift=-1.0cm, yshift=0.8cm]{d};
        \node[font=\rmfamily,yshift=0.8cm, xshift=0.55cm, anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c} Filter coefficients  {\color{mplGreen}$\beta_{\theta}$}\\ with p-values $\ge0.05$\end{tabular}}};
        \node[xshift=0.35cm, yshift=0.2cm]{\includegraphics[scale=0.07]{figures/filter.png}};
    \end{scope}

    \begin{scope}[xshift=5.8cm] %Big contribution
        \node[roundnode, xshift=-1.05cm, yshift=0.8cm]{c};
        \node[font=\rmfamily,yshift=0.8cm, xshift=0.55cm, anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c} Find largest coefficient \\for each feature $j$\end{tabular}}};

        \begin{scope}[xshift=0.3cm]
        \node[font=\rmfamily,yshift=-0.35cm, xshift=-0.0cm, anchor=south]{
        \setlength\tabcolsep{0.pt}%
        \fontsize{8}{8}\selectfont{\begin{tabular}{rl} {
        $($\color{mplGreen}$\beta_{\theta^j}^{j}$}$)^2$&$=(${\color{mplBrown}$\beta_{0\degree}^{j}$}$)^2+(${\color{mplCyan}$\beta_{90\degree}^{j}$}$)^2$  \vspace{0.14cm} \\
        % $\theta^j$ &$= \argmaxF_\theta \beta^j$ \\[-0.07cm]
        $\theta^j$&$= \arctan(${\color{mplCyan}$\beta_{90\degree}^{j}$}$ / ${\color{mplBrown}$\beta_{0\degree}^{j}$}$)$  
        \end{tabular}}};

        \begin{scope}[scale=1.6, xshift=1.2cm, yshift=-0.1cm]
            \draw [gray,-{Latex[length=1.5mm]}, line width=0.2mm] (-0.1,0) -- (0.9,0);
            \draw[gray,-{Latex[length=1.5mm]}, line width=0.2mm] (0,-0.1) -- (0,0.6);

            \draw [gray,dotted, line width=0.16mm] (0,0.4) -- (0.7,0.4);
            \draw[gray,dotted,line width=0.16mm] (0.7,0) -- (0.7,0.4);
    
            \draw[mplCyan,-{Latex[length=2mm]}, line width=0.5mm] (0,0) -- (0,0.4);
            \draw[mplBrown, -{Latex[length=2mm]}, line width=0.5mm] (0,0) -- (0.7,0.0);
            \draw[mplGreen, -{Latex[length=2mm]}, line width=0.5mm] (0,0) -- (0.7,0.4);

            \draw[thick, ]
            (0.2296,0) .. controls (0.2277,0.0519)..
            (0.1890,0.0945);
            \node[anchor=west] at(0.3277,0.119){\fontsize{8}{8}\selectfont{$\theta^j$}};

            \filldraw[gray, fill=none] (0.35,0.2) circle (0.4);
            
        \end{scope}
        \end{scope}
    \end{scope}

    \begin{scope}[xshift=13.0cm, yshift=0.3cm] %Clock
        \node[xshift=0.35cm]{\includegraphics[scale=0.8]{figures/pima_only_clock.pdf}};
        \node[font=\rmfamily,yshift=0.8cm, xshift=0.35cm, anchor=south]{\fontsize{8}{8}\selectfont{\begin{tabular}{c} \textbf{Feature Clock}\end{tabular}}};
        \node[roundnode, xshift=-0.7cm,yshift=-1.1cm]{e};
    \end{scope}

    
    \begin{scope}[on background layer] %Box
        \node[fill=white!90!mplCyan, minimum height=2.3cm, minimum width=11.6cm,xshift=6.2cm, yshift=0.5cm,rounded corners=0.5cm]{};
    \end{scope}

\end{tikzpicture}

\vspace{-0.30cm}
\caption[teaser]{Feature Clock uses {\nodeLabel{a}} high \textbf{X} and low \textbf{Y} dimensional data.~\nodeLabel{b} 
We define the feature contribution as a coefficient of the linear regression (LR) between \textbf{X} and $\mathbf{y_\theta}$ (\textbf{Y} projected at angle $\theta$). The optimization goal is to find the angle $\theta^j$ at which the coefficient $\beta_{\theta^j}^j$ of feature $j$ is maximized. \nodeLabel{c} The solution is derived from LR coefficients of $\theta=0\degree$ and $\theta=90\degree$.~\nodeLabel{d} We filter the insignificant LR coefficients based on p-values. Features with insignificant p-values are not visualized.~\nodeLabel{e} The largest coefficient of each feature is visualized in the Feature Clock.}
\label{fig:teaser}


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> methods_old.tex <==
\section{Methodology}
\label{Methods}

In this section, we outline the internals of the Feature Clock.
The general functionality of the Feature Clock library is shown in~\cref{fig:teaser}. 

Before the plotting, the high- and low-dimensional data are pre-processed, and the latter is projected on the x- and y-axis.
% The projections are used in all three visualizations.
In the data preparation, both high- and low-dimensional data are optionally standardized with standard score normalization for each column. 
% The standardization ensures the errors are normalized for the subsequent linear regressions.

% \begin{figure}[t]
% \vspace{-1em}
% \begin{algorithm}[H]
%     \caption{Clock Algorithm Outline.}\label{alg:outline}
%     % \small
% \setlength{\textfloatsep}{0pt}
%     \begin{algorithmic}
%         \Require{High-Dim: $\mat{X}$, Low-Dim: $\hat{\mat{X}}$, Selection: $\mat{s}$}

%         \noindent
%         \State $\mat{X},\hat{\mat{X}} \gets \textsc{preprocess}( \mat{X},\hat{\mat{X}} ) $
%         \State $\mat{C} \gets []$
%         \For{ $r$ \textbf{in} $[0\degree, 90\degree]$}
%             \State $PF_r \gets \textsc{project}(\hat{\mat{X}},r)$
%             \State $\mat{C}_r \gets \textsc{linearRegression}(\mat{X}, PF_r)$
%             \State $\mat{C}_{sr} \gets \textsc{filter}(\mat{s}, C_r)$
%             \State $\mat{C} \gets \textsc{append}(\mat{C}, \mat{C}_{sr})$
%         \EndFor
%         \State $\mat{C}_m \gets \textsc{maxContribution(\mat{C})}$
%         \State $\textsc{plotClock}(\mat{C}_m)$
        
%     \end{algorithmic}
    
% \end{algorithm}
% \vspace{-3em}
% \end{figure}

% \subsection{Feature Clock}

\textbf{Feature Clock Overview:}\label{sec:feature-clock}
We project the low-dimensional data (e.g., UMAP 2D data) on the x- and y-axis, this can be interpreted as a projection on the radius of the semicircle at $0\degree$ and $90\degree$ angles.
For each projection, we rotate the axis of the 2D coordinate system by $0\degree$ and $90\degree$ such that all projected low-dimensional points lie on the x-axis with a zero y coordinate.
In this case, projection and rotation are equivalent to taking x and y of low-dimensional data, but it is an important step for the later understanding of the method.
We store the x coordinate of each point for each angle as an \emph{projection factor} (PF). 
The PF defines how each point contributes in a certain direction.% of the x- and y-axis.
% 
To find the contribution of high-dimensional features in the low-dimensional space, we fit a multivariate linear regression (LR) model for each PF (one LR for x, another for y low-dimensional values).
% (one LR for $0\degree$, another for $90\degree$)
The input of the LR is the high-dimensional data, $X$, and the dependent vector $d$, the PF.
% of selected features in a particular direction.
Each LR produces a coefficient $\beta_{\theta}^j$ and a p-value for each feature, and the insignificant features are filtered out (p-value $> 0.05$ for both $0\degree$ and $90\degree$). 
% The impact of filtered-out values is neglected since their contribution is almost zero.
% If there are no significant variables, then the clock is not visualized. 
The LR coefficients of the remaining features are used as the magnitude of the impact of high-dimensional features.
The coefficients are optionally standardized using standard deviation.
To find the biggest impact of a feature from just two LR coefficients, we utilize some geometrical properties explained in~\cref{sec:supplemental_materials}.
We define the biggest contribution of each feature $j$ using two LR coefficients, $\beta_{0\degree}^j$ and $\beta_{90\degree}^j$.
The biggest impact vector has coordinates $\left\langle (0,0), (\beta_{0\degree}^j, \beta_{90\degree}^j)\right\rangle$ on the circle.
A formal proof is included in the Supplemental Material.
% The $x$ and $y$ coordinates of features' biggest impact vector are coefficients of a respective feature.
% 

\input{figures/semicircleTikz}

\begin{figure*}[!t]
    \vspace{-0.5cm}
    \centering\begin{tikzpicture}
        \node{
            \includegraphics[width=\linewidth]{figures/support_3.jpg}
        };
        \node at (-8.72cm,1.0cm){{a}};
        \node at (-4.23cm,1.0cm){{b}};
        \node at (0.26cm,1.0cm){{c}};
        \node at (4.75cm,1.0cm){{d}};
    \end{tikzpicture}
    \vspace{-0.7cm}
    \caption{(a) Global Feature Clock shows the general trend for top-4 significant features, while (b) scatter plots support the Global Clock and show the value range of top-4 high-dimensional features for hospital survival. (c) Local Clocks help to inspect the data within original labels (patient survived/died in hospital) while (d) Inter-group Clock shows how features change between two classes.}
    \label{fig:supportClocks}
    \vspace{-0.5cm}
\end{figure*}

An alternative to visualizing one coefficient per variable is to project low-dimensional data on the radius of the semicircle at different angles, see~\cref{fig:semicircleProjection}, and visualize all coefficients for all features per projection, see~\cref{sec:supplemental_materials}. 
This results in perfect circles that appear because of projecting and rotating.
Projection angles are defined by incrementing from $0\degree$ to $180\degree$ by a user-defined $\theta=\frac{180\degree}{\mat{n}}$ with n projection lines, where $\theta=5\degree$ is the default value. 
We have experimented with different $\theta$ values, and smaller $\theta<5\degree$ do not lead to a better human perception, while the bigger $\theta$ the fewer regression models should be fitted.

We default to plot the largest coefficient since it leads to a cleaner visualization while maintaining maximum information, but the user can opt for the "circles" visualization.
% The magnitude of the largest coefficient is defined by its value. 
The plot is easily interpreted, the vector length encodes feature impact in the given direction for the selected points.  
If dataset has many features, user can visualize only top-$k$ variables with the biggest impact and are selected automatically.
We place the clock in the center of the low-dimensional points.
The location does not influence the clock construction.

%\subsection{Global Clock}
% \noindent
\textbf{Global Feature Clock:} We construct a clock using all data points to visualize the impact of the high-dimensional features in the latent space.
The Global Clock shows the general value alternation of the high-dimensional features.
The disadvantage of the Global Clock is that it does not capture finer changes of gradients across the whole data, but rather a general trend. 
Since we approximate the path on a manifold with a line, a clock can miss some information.

%\subsection{Local Clocks}
% \noindent
\textbf{Local Feature Clock:}
We use a Local Clock technique to explore data at the finer granularity. The Local Clocks take a selection of points for analysis and enable easier analysis of neighboring points. A user can explore how different features change within a group.
Class labels or clustering of high-dimensional data determine the points used for a single clock.
Analyzing original labels gives a perspective on what drives particular classes, while clusters help to understand the latent space made by nonlinear dimensionality reduction. 
We default clustering to HDBSCAN, but a user can define own clusters via any clustering algorithm.
Importantly, HDBSCAN also identifies outliers that are not assigned to any cluster.
% Interestingly, HDBSCAN clusters of high-dimensional data correspond to the embeddings computed by NLDR.
For each cluster or class, we apply the same method as in~\cref{fig:teaser} and create a single clock signifying changes within selected points.

%\subsection{Inter-group Clock}
% \noindent
\textbf{Inter-group Feature Clock:}
We have opted for a third visualization to inspect how variables change between groups, either classes or labels.
To analyze the relationship between the two groups, we apply logistic regression.
We fit a binary classifier with the high-dimensional observations from two groups and visualize statistically significant coefficients for a single line that connects the group centers.
The result is a single line that signifies the most influential high-dimensional features between the groups.
In a multi-group setting, there is a space limitation for plotting all pairs of groups and their clocks.
Therefore, we build a minimum spanning tree (MST) between group centers in low-dimensional space and plot the inter-group relationships for all MST edges.
A clock on each edge of MST shows the feature impact between groups.

\textbf{Limitations:} 
We explain high-dimensional contributions with linear directions.
If data is dense, we can approximate the movement of the gradients on the manifold in the original high-dimensional space with the shortest distance on average in low-dimensional space~\cite{Cheng2013HW}.
We assume that the shortest path is a line.
In the nonlinear-dimensionality reduction, a heavy-tailed distribution is used to measure similarities between points to allow dissimilar objects to be modeled far apart in the map~\cite{tSNE}.
If points are sparse, they end up in the tail of the distribution and have insignificant effect~\cite{wattenberg2016how}.
The three suggested visualizations advise a user about high-dimensional data. 
Generally, some information might be missed since we might not follow the actual manifold and an exact path on it.
Another downside of the clock is that we can not see all contributions if they overlap and are of the similar size.
In the Inter-group Clock, visualization of all contributions on a single line leads to the overlay of multiple vectors that are potentially of the same magnitude.

\textbf{Example:} \textit{\cref{fig:biplot} shows a PCA biplot with feature loadings, t-SNE scatter plots for each variable, and Feature Clock for the Iris dataset~\cite{IrisData}.
Byplot (\cref{fig:biplot}a) shows how features influence low-dimensional representation.
We can see that petal width and length are the driving factors for the versicolor and verginica classes.
The scatter plots, in~\cref{fig:biplot}b, display how high-dimensional values of each feature are distributed in the t-SNE latent space.
% The values increase with the x coordinate. 
All features except sepal width increase the most with increasing x and y values.
Finally, from a Feature Clock in~\cref{fig:biplot}c, we observe how each variable impacts t-SNE embedding.
In the Feature Clock, for t-SNE, sepal length is insignificant, while petal length is a driving factor.
Also, sepal width influences setosa class, similarly to the PCA.
% We can see that in t-SNE latent space, all three classes are almost linearly separable, while this is not the case for PCA.
}

